Fine-Tuning Language Models on Multiple Datasets for Citation Intention Classification

Citation intention Classification (CIC) tools classify citations by their intention (e.g., background, motivation) and assist readers in evaluating the contribution of scientific literature. Prior research has shown that pretrained language models (PLMs) such as SciBERT can achieve state-of-the-art performance on CIC benchmarks. PLMs are trained via self-supervision tasks on a large corpus of general text and can quickly adapt to CIC tasks via moderate fine-tuning on the corresponding dataset. Despite their advantages, PLMs can easily overfit small datasets during fine-tuning. In this paper, we propose a multi-task learning (MTL) framework that jointly fine-tunes PLMs on a dataset of primary interest together with multiple auxiliary CIC datasets to take advantage of additional supervision signals. We develop a data-driven task relation learning (TRL) method that controls the contribution of auxiliary datasets to avoid negative transfer and expensive hyper-parameter tuning. We conduct experiments on three CIC datasets and show that fine-tuning with additional datasets can improve the PLMs' generalization performance on the primary dataset. PLMs fine-tuned with our proposed framework outperform the current state-of-the-art models by 7% to 11% on small datasets while aligning with the best-performing model on a large dataset.

==> Sections/Abstract.tex <==


% Citation intention identification (CII) tools classify citations by their intention (e.g., background, motivation) and assist readers in comprehending scientific literature. Prior research has shown that pretrained language models (PLMs) such as SciBERT can achieve state-of-the-art performance on CII benchmarks. PLMs are trained via self-supervision tasks on a large corpus of general text and can quickly adapt to CII tasks via moderate fine-tuning on the corresponding dataset. Despite their advantages, PLMs can easily overfit small datasets during fine-tuning. In this paper, we propose a multi-task learning (MTL) framework that jointly fine-tunes PLMs on a dataset of primary interest together with multiple auxiliary CII datasets to take advantage of additional supervision signals. We develop a data-driven task relation learning method that controls the contribution of auxiliary datasets to avoid negative transfer and expensive hyper-parameter tuning. We conduct experiments on three CII datasets and show that fine-tuning with additional datasets can improve the PLMs' generalization performance on the primary dataset. Our proposed MTL fine-tuning framework outperforms the current-state-of-the-art models by 1.3 to 5.0 in absolute macro-F1 scores on the three benchmark datasets.

Citation intention Classification (CIC) tools classify citations by their intention (e.g., background, motivation) and assist readers in evaluating the contribution of scientific literature. Prior research has shown that pretrained language models (PLMs) such as SciBERT can achieve state-of-the-art performance on CIC benchmarks. PLMs are trained via self-supervision tasks on a large corpus of general text and can quickly adapt to CIC tasks via moderate fine-tuning on the corresponding dataset. Despite their advantages, PLMs can easily overfit small datasets during fine-tuning. In this paper, we propose a multi-task learning (MTL) framework that jointly fine-tunes PLMs on a dataset of primary interest together with multiple auxiliary CIC datasets to take advantage of additional supervision signals. We develop a data-driven task relation learning (TRL) method that controls the contribution of auxiliary datasets to avoid negative transfer and expensive hyper-parameter tuning. We conduct experiments on three CIC datasets and show that fine-tuning with additional datasets can improve the PLMs' generalization performance on the primary dataset. PLMs fine-tuned with our proposed framework outperform the current state-of-the-art models by 7% to 11% on small datasets while aligning with the best-performing model on a large dataset.

==> Sections/Model.tex <==
% Put an overview of our proposed methods, and our novel components in the framework here.

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{Figures/DeepCiteVer1.pdf}
\caption{Overview of the architecture of our multi-task learning framework. The top portion depicts our three pooling operations (cls, mean, citation token) over the language model embeddings to generate the representation for the citation context. The bottom portion depics the multi-head structure, each task has a seperate MLP layer for prediction. The same language model parameters are shared across all tasks.    
% Pre-trained language model for citation intention identification and the multi-task fine-tuning framework.
}
\label{fig:DeepCite}
\end{figure*}

We use a pre-trained language model as the text encoder that converts citation contexts to vectors in a latent space and multi-layer perceptrons (MLP) as classifiers to map the vectors to logits over intention labels. We use transformer-based~\cite{vaswani2017attention} PLMs, e.g., BERT~\cite{devlin2019bert} and SciBERT~\cite{beltagy2019scibert}, as they are the \textit{de facto} standard language models nowadays.

PLMs output one contextualized embedding for each position of the text input. A readout function is needed to compress the embedding matrix to a fixed size vector to feed into the downstream MLPs. One critical feature of citation intention identification (CII) tasks is that their input, citation context, contains not only a snippet of text but also the position of the citation which is helpful for predicting the function of the citation. Existing methods for text classification tasks usually use the output embedding of a special token (i.e., [CLS]) or the average pooling of all embeddings to be the text representation \cite{beltagy2019scibert, devlin2019bert, reimers2019sbert}. Although these readout methods achieve satisfying performance in general text classification tasks, they are sub-optimal for CII tasks as they are agnostic of the citation position. 

We develop a position aware readout function for CII tasks. We insert a special mark <CITED HERE> into the position of the citation in the context, and use the embedding of the mark to be the representation of the citation to feed into MLPs (see an example in Figure~\ref{fig:DeepCite}). Our experiments in Section~\ref{sec:readout} show that this readout method outperforms position agnostic readout functions.


% Split the whole framework into several sections. The first section should be an illustration of the general method (use (Sci)BERT + MLP for intention classification). The other sections should be our novel components, two multi-task learning methods, how we readout, our ways to include extra information (title, abstracts).

% \subsection{Context Featurization}

% Context featurization, i.e., convert an irregular shaped text input, citation context(s), to a fixed length contextualized vector, is a core step in citation intention identification (CII) tasks. 

% PLMs can usually takes 

==> Sections/Motivation.tex <==
% The objective of this work is to evaluate the performance of multi-task learning using pre-trained language models for the problem of CII classification on domain specific datasets for which limited training samples are available.  Specifically, we seek to accurately predict the citation intent for papers sourced from the Knowledgebase of Interatomic Models (KIM)\footnote{\url{https://openkim.org/}} project \cite{kim2011}.  The KIM project is an NSF-funded cyberinfrastructure that archives empirical interatomic models\footnote{An \emph{interatomic model} is a computational algorithm that given the positions and chemical elements of a set of atoms, returns the energy and forces on the atoms.} that are used by molecular simulation codes to predict the behavior of materials and nanosystems based on their atomic structure.  Each interatomic model in the KIM repository is accompanied by metadata that includes the primary literary work(s) in which the model was first published.  Profiling the body of citing content in the literature is useful because it aids in model selection, i.e.\ the process of selecting a model from the KIM repository for a specific scientific application.  First, the overall number of citations that a model has garnered over time is an indication of its utility across a broad range of applications, at least insofar as its basic formulation is concerned.  By identifying which citing papers actually used the model, as opposed to those which cite it only for general context, and parsing their contents to identify the application(s) studied within, further knowledge can be gleaned as to the model's domain of applicability.  Combining such information for the entire body of models in the KIM repository provides a means for a user to identify the set of all models for a given material system that have been used for a specific application.

The objective of this work is to enhance the performance a small, domain specific CII classification dataset by leveraging existing larger scaled CII datasets. Curating a domain specific dataset is a time consuming process that requires experts in the field to analysis. In this work our primary dataset of interest was created from the Knowledgebase of Interatomic Models (KIM)\footnote{\url{https://openkim.org/}} project \cite{kim2011}. KIM archives empirical interatomic models\footnote{An \emph{interatomic model} is a computational algorithm that given the positions and chemical elements of a set of atoms, returns the energy and forces on the atoms.} that are used by molecular simulation codes to predict the behavior of materials and nanosystems based on their atomic structure. Domain experts annotated citations of interatomic models listed on KIM across 614 papers. This resulted in a dataset with 804 samples.  
